Advanced Manufacturing Configuration by Sample-efficient Batch Bayesian Optimization

We propose a framework for the configuration and operation of expensive-to-evaluate advanced manufacturing methods, based on Bayesian optimization. The framework unifies a tailored acquisition function, a parallel acquisition procedure, and the integration of process information providing context to the optimization procedure. \cmtb{The novel acquisition function is demonstrated, analyzed and compared on state-of-the-art benchmarking problems. We apply the optimization approach to atmospheric plasma spraying and fused deposition modeling.} Our results demonstrate that the proposed framework can efficiently find input parameters that produce the desired outcome and minimize the process cost.

==> Reviews/Answer_to_reviewer_11.tex <==
\textbf{\large Reply to Reviewer 11:}\\\\
We thank the reviewer for their evaluation, comments, and suggestions on improving the quality of the manuscript.\\  


%----------------------------------------------------------------------
\textbf{Comment 1:}
The paper is probably publishable, but should be reviewed again in
revised form before it is accepted.
A GP model structure is used to predict coating properties in this
paper, and an algorithm is proposed to enhance reproducibility in
realtime process measurements. The experimental results the proposed
method can efficiently find good configuration of APS process. The
article is well organized and its presentation is good, and the
citations is adequacy. However, some minor issues still need to be
improved.

\textbf{Reply:}
We thank the reviewer for their comments on organization, presentation and citations.\\

\textbf{Comment 2:}
In the present work, Gaussian process regression (GPR) is used to
predict coating properties, its high computational complexity of both
large data points and high dimension (using all variables in Section of
Method) limits the real-time application. An explanation of your
tractable computation power should be provided. 

\textbf{Reply:}
We agree on the fact that Gaussian process models can become extremely expensive in terms of computational time and thus make real-time applications impossible. However, in the context of Bayesian optimization this is rarely an issue. The goal of our Algorithm is to use as few samples as possible, keeping the data set size small and thus the GPs models easily usable. Additionally, we do not really require a real-time application: we conduct the process modeling and optimization in between two batches of experiments and have as much time as needed to do so. In reality, the algorithm code takes a couple of minutes to run on a standard laptop even with the largest available data set. This time is substantially smaller than the time needed to set-up the industrial equipment for another batch (approx. one day). We have clarified this point, in section \ref{sec_model_structure}.\\

\textbf{Comment 3:}
There is a lack of the explanation of whether collected training data
set are able to cover regression feature-space effectively? If it is
ineffective, the generalization ability is limited without high
accuracy of prediction for those sufficient distant data points.

\textbf{Reply:}
We thank the reviewer for raising this point. More information on it is provided in section \ref{data_coll}. Fractional factorial design allows to effectively expose the most important features of the process while reducing the effort/cost of a full factorial experiment. This is particularly useful in the context of our application, where each experiment is extremely time consuming and expensive. The amount of levels at which the inputs where set were selected by APS experts based on their knowledge of the process and its behavior. This guarantees that the feature space is covered in an effective manner.\\

\textbf{Comment 4:}
In the subsection of Modeling Validation, an explanation of why the
selected five combinations have the highest confidence should be
provided.

\textbf{Reply:}
We appreciate this question and understand that the sentence formulation was probably misleading. We have now modified section \ref{sec_mod_res} to make it clearer. We select the five combinations that -- after model training -- are far enough from training inputs and have the lowest GP posterior variance. This means that we select the points in which our models show the lowest learning error (i.e. the highest confidence).

==> Reviews/Answer_to_reviewer_15.tex <==
\textbf{\large Reply to Reviewer 15:}\\\\
We thank the reviewer for their evaluation as well as their comments and suggestions on improving the quality of the manuscript.\\  


%----------------------------------------------------------------------
\textbf{Comment 1:}
This paper presents an application of constrained BO to tune atmospheric plasma spraying, an expensive-to-evaluate industrial process. The cost function to minimise in this case has a known
deterministic form. However, the constraints related to coating limits
are expensive to evaluate. The proposed approach includes the
derivation of two new acquisition functions tailored for these settings
of a known-objective with black-box constraints. Experimental results
with synthetic and real data are presented.\\
Applying BO to real-world problems often requires adaptations to make
methods more efficient in problem-specific settings. This paper
presents the case of an industrial application with processes which are
inherently noisy and expensive to evaluate, as BO methods are usually
motivated towards. The paper is also mostly well written and follows a
clear structure. However, there are a few issues in its current form,
which might make it not suitable for publication. I elaborate on them
below.

\textbf{Reply:}
We thank the reviewer for the precise summary and for their comments on the writing style and structure.\\

\textbf{Comment 2:}
Experiments provide no comparisons against baseline methods. The
modelling component of the proposed framework is assessed in terms of
predictive power against real data. The optimisation component,
however, an essential part of the paper's main contribution is not
compared against other methods. Therefore, it is hard to judge whether
the proposed BO framework offers real performance improvements against
existing out-of-the-box constrained BO methods (e.g., \cite{Gardner2014BayesianConstraints}).

\textbf{Reply:}
We agree with the reviewer on the fact that the optimization is a central component of our work, and having an experimental comparison with another method would have been beneficial.
The limited amount of possible experiments -- due to the cost and characteristics of the APS process -- is the reason why we were not able to achieve it, and it is also the reason why we choose batch Bayesian optimization. Not only the cost of each conducted experiment is extremely high, but the time required to set-up, conduct and then analyze a batch of experiments is approximately 3 to 4 months. As detailed in our work, these time constraints limited the experimental evaluation to only the first batch of the optimization process. We chose on purpose not to compare it \emph{experimentally} with other out-of-the-box CBO methods such as \cite{Gardner2014BayesianConstraints} as in the first batch no difference would have been visible: during the initial search -- when no feasible point is known -- both methods select candidates by maximizing their probability of feasibility. We now include a comparison in \emph{simulation} (the results are summarized in Table \ref{tab_comparison}, also relevant to the next comment). Specifically, in the last column of Table \ref{tab_comparison}, where the acquisition function is \textit{constrained expected improvement}, the comparison is provided in terms of number of experiments and batches needed to reach convergence of the algorithm according to the provided stopping criterion and shows that the proposed method is more efficient and achieves convergence in a smaller number of experiments.
\\

\textbf{Comment 3:}
One could argue that experimental comparisons using the real APS
system are too expensive to run, so that the results in Sec. \ref{sec_exp_opt} are
still acceptable. However, the numerical experiments in Sec. \ref{sec_simulated_res} were
performed using a neural network oracle, which should much cheaper to
evaluate, allowing for comparisons against other BO methods as
baselines.

\textbf{Reply:}
We sincerely thank the reviewer for this contribution regarding the possibility to conduct comparisons in the simulated case.
We have conducted simulated comparisons between our proposed method, its individual components and the BO method that has been successfully applied to industrial applications \cite{Gardner2014BayesianConstraints}. The comparisons are summarized in Table \ref{tab_comparison} and commented in section \ref{sec_simulated_res}. The results show that a combination of acquisition functions, as proposed in the paper, achieves the smallest number of experiments.
\\

\textbf{Comment 4:}
There is some missing detail about the modelling of the constraints.
Are each of the constraints ($c_1$ and $c_2$) modelled with an independent
GP? Or are they jointly modelled by a vector-valued GP?

\textbf{Reply:}
We appreciate the question, and have clarified in the text the modeling of the constraints. All modeling has been conducted with independent GPs. This applies to all four coating quality parameters, including the two that have been selected as constraints ($c_1$ and $c_2$). We have added one sentence that clarifies this in section \ref{sec_model_structure}.\\

\textbf{Comment 5:}
Some symbols are left undefined in Algorithm \ref{alg_workflow}: e.g. $\textbf{y}$
(constraint evaluations?), $\mu_\textbf{c}$ (predictive mean
of the constraints?)

\textbf{Reply:}
The notation had been chosen for the sake of brevity and we agree that it lacked in clarity. The bold letters indicate a  collection of multiple scalar values in the case where multiple constraints are being evaluated for a certain candidate. Thus, $\textbf{y}$ collects $y_1$ and $y_2$ and $\mu_\textbf{c}$ groups $\mu_{c_1}$ and $\mu_{c_2}$, the predictive means of the constraints $c_1$ and $c_2$. We have chosen not to base the Algorithm explicitly on $c_1$ and $c_2$ as any number of constraints can be used. We have added the required clarifications and definitions Algorithm \ref{alg_workflow} text.\\

\textbf{Comment 6:}
The threshold $\pi$ should be in the interval [0,1], but this is not
explicitly mentioned with its definition under Eq. 5b.

\textbf{Reply:}
We thank the reviewer for this remark. We have added this important condition to the definition of $\pi$ in section \ref{sec_acquisition_procedure}.\\


\textbf{Comment 7:}
$\Sigma$ is usually the symbol for a covariance matrix.
However, it's apparently being used in Sec. III as the GP std.
deviation, which is somewhat confusing, as it is a scalar. If that's
the case, $\sigma$ would be a better notation.

\textbf{Reply:}
Indeed, we agree with the proposed change in notation. We have modified the notation of section \ref{sec_GP} according to the comment, as we are indeed looking at the GP posterior standard deviation.

==> Reviews/Answer_to_reviewer_17.tex <==

\textbf{\large Reply to Reviewer 17:}\\\\
We are grateful to the reviewer, their evaluation as well as their valuable comments, questions, and suggestions on improving the quality of the manuscript.\\  


%----------------------------------------------------------------------

\textbf{Comment 1:}
First off, I love the application of Bayesian optimization (or, more generally, intelligent design of experiments) to another new field/topic.  I think that the authors have worked to achieve the hardest part of the adaptation process required to leverage advanced modifications of BO in previously uncharted territory. ...I would like to start this by saying that I enjoy the novelty of your acquisition function.

\textbf{Reply:}
We thank the reviewer for the positive feedback.\\
 
\textbf{Comment 2:} 
It is not obvious to me what this paper is trying to achieve.  On one hand, I think the authors argue that they are trying to build a Gaussian process modeling strategy specific to their problem, as well as an acquisition function better suited to their specific form of constrained BO.  That is good, I like that -- but then the strategy that you used and the results of your paper are only relevant to your exact problem (which is so secretive that you couldn't even explain completely what it is).

\textbf{Reply:}
We appreciate this comment. We have now clarified in the paper that the method is applicable to more than one specific problem. We have restructured the paper to make this clearer. Now, the batch-BO method is presented first, independently from the plasma spraying process, and the modeling and results demonstrated for this particular process are presented afterwards. 
In particular, the method can be applied to various manufacturing processes which are complex to conduct, expensive, slow, or require expensive evaluation to asses the achieved quality. Such processes are other types of plasma spray coating -- such as VLPPS (very low pressure splasma spray) -- or additive manufacturing processes (selective laser melting, wire arc additive manufacturing, etc). The method's main benefit is that it achieves favorable configurations of parameters much faster than other methods, including those based on BO. This makes it possible to enable manufacturing of very small lots, without extensive simulations, time and experiments optimizing for the best parameters, which is one of the main goals in intelligent manufacturing. We have addressed these points in the introduction and, in particular, in the contributions of the paper. We believe this rearrangement and clarification has increased the value of the paper, and are very grateful to the reviewer for pointing this out.\\


\textbf{Comment 3:}  I have no perspective of the significance of the modeling results presented in Figures \ref{fig_exp_val} \& \ref{fig_mhard_drift},
nor the BO results presented in Figures \ref{fig:detailed_opt} \& \ref{fig_experimental_opt}. Frankly, I don't know what fraction of the RA-L audience is going to understand how difficult it is to achieve your goal to "find combinations of inputs producing coatings with microhardness ranging between 635HV and 675HV and porosity between 6\% and 8.2\% while minimizing the gun stress index."  And you do not present any competing methods to provide a frame of reference for readers.

I can be okay with the idea that the application is just a motivation and your real contribution is the algorithm.  But I see two fundamental problems with how you have executed on this front.  First, the algorithm is never compared against any alternatives, or even on any problems that anyone else in the world can run (given your
confidentiality).  How can the significance of your work be judged in such a vacuum? Second, you have done a significant amount of work to develop modeling strategies which are, possibly, only relevant for this specific application.  If you want to argue that there is an algorithmic contribution, don't you need to test this algorithm more broadly and see when it performs well and when it does not?

Essentially, my main problem is that this article wants to focus on a specific application but is trying to present a result as being more general than is demonstrated.  Either a number of more general tests need to be run to make an actual statement about your algorithm, or you should publish this in a forum where people can understand your
application, and then more specifically explain the significance of this previously unachieved performance.

\textbf{Reply:}
We appreciate this comment. Indeed, the main contribution of the paper is the presented algorithm. We have rearranged the paper to highlight this contribution. We have modified the structure of the paper, the introduction, and the contribution description to make it more clear. The method is presented independently first, and then demonstrated in the plasma spraying process parameter optimization.
We have now included a comparison with other BO-based methods is simulation (the results are summarized in Table \ref{tab_comparison}). This was not possible to do experimentally, as the time required to set-up, conduct and then analyze a batch of experiments is approx. 3 to 4 months. This comparison shows that our method (Table \ref{tab_comparison}, column 1) performs better than simply conducting BO with one acquisition function (columns 2, 3), as well as better than the standard constrained BO (column 4).
The comparison is made in terms of number of experiments and batches needed to reach convergence of the algorithm according to the provided stopping criterion and shows that the proposed method is more efficient and achieves convergence in smaller number of experiments. \\


\textbf{Comment 4:}  The results in Figure \ref{fig_exp_val} seem a bit troubling to me. First, you said that you created 86 pieces of data for your training set and 23 pieces of data for your validation set.  When I look at the Porosity graph, I
count only 15 red squares.  Am I misunderstanding where the 23 is being used, or are there just some squares that happen to lie exactly on top of each other?	If there are, that seems a bit odd, right, given your statement in Table II about how much noise is affecting the accumulation of data?

\textbf{Reply:}
We thank the reviewer for spotting a small mistake in the function that generated the plot of Fig. \ref{fig_exp_val}. The content of the figure has now been updated to include the eight baseline runs that were erroneously omitted. All 23 validation experiments are now correctly shown.\\

\textbf{Comment 5:} Beyond that, I am very concerned about the distribution of the Validation values relative to the Training values.  When I think about the training/validation split in surrogate modeling, I think that the goal is for the training and validation sets to somehow be drawn from the same distribution. The fact that the red squares seem to occupy only a fraction of the region that the blue dots occupy makes me worried that they do not belong to the same distribution.  As a result, it makes me somewhat concerned about how effective these GP models are, and in turn how much your algorithm actually relies on them (assuming the algorithm is performing well). 
Your strategy for creating this validation set was arbitrary, and not at all reproducible (given the expertise required), so this is part of my concern about suggesting a significant algorithmic novelty in this article.

\textbf{Reply:}
We appreciate this remark, and have addressed it in the paper. Indeed, the training/validation split is not ideal in terms of distribution. This is due to the experimental context in which we worked. The high cost of data collection forced us to operate budget aware choices when designing the validation experiments. Thus, we based our decisions on the expertise of the people that have been working industrially with the APS process for years and focused on only one of the two powders that were used for training. This powder is considered harder to model and produces results in the high microhardness/low porosity region. We have tried to clarify this in section \ref{data_coll}.

Additionally, we would like to highlight the fact that the models have higher performance when creating and aggregate data set (86+23 samples) and then splitting it randomly for cross-validation. This is however a much simpler task, given the nature of our problem. The main challenge in this class of problems is given by the unknown and uncontrollable change in equipment status between different experimental sessions, which is inherent to a production plant. This is why training on a data set collected entirely in one session and validating on the data belonging to another session is a task that needs to be addressed - it is also the most realistic scenario that happens in practice. Given the restricted amount of data that we could collect and the choices that we had to operate, we believe that the presented validation set is the most effective in highlighting the models performance. This has been clarified in section \ref{sec_mod_res}.\\

\textbf{Comment 6:}
Along these lines, I worry about this voltage discussion. First, Figure \ref{fig_mhard_drift} seems to present a bizarre disconnect between the training and validation data; why did you use totally different methods to create the training and validation datasets?  Why not use the exact same strategy for both?  Second I can read the Section \ref{sec_opt_workflow} and somewhat
understand how you are incorporating voltage, but not really. And it should not matter if the focus is on the algorithmic side (since this strategy would not be applicable in any other settings).  The comment "voltage cannot be ... optimized" feels false as well.	If I understand, voltage is a function of your tunable parameters.  How would optimizing it be any different than optimizing any other black-box function (which is what BO is built to do)? 

\textbf{Reply:}
We thank the reviewer for raising this point. We have modified the comment to Fig. \ref{fig_mhard_drift} to clarify its content. What we want to show is that we observe an offset in the output properties achieved in baseline runs in different experimental sessions. From session to session, the input parameters in these baseline runs do not change. However, the achieved output quality parameters show a clear offset. For example, in Fig. \ref{fig_mhard_drift}, the average microhardness of the training baseline samples (coated in the first session) is approx. \SI{525}{HV}. However, the microhardness of the validation samples (coated a second session) is approx. \SI{625}{HV}. This offset is caused by a change in the equipment status (e.g. aging, wear and tear, maintenance etc.) that makes it impossible to produce coatings with identical properties in different sessions (as discussed as well in the previous comment). 
The measured gun voltage cannot be tuned directly as it depends on the unknown equipment status, and it is not one of the parameters that are used to set-up and control the process, in contrast to current, gas flow rate, etc.
Figure \ref{fig_mhard_drift} shows that this voltage is correlated with microhardness (a property that we want to control and maintain within certain constraints). We propose to use this voltage measurement as an indication for the equipment status to address the issue of session-to-session lack of reproducibility. We have modified section \ref{sec_opt_workflow} to clarify how we are using status dependent measurements (such as voltage) to anticipate the changes in output properties that the equipment status causes.\\

\textbf{Comment 7:} In your abstract you claim "We ... propose an algorithm that adapts to real-time process measurements to improve reproducibility."	I do not feel that you have done that anywhere in the paper.  I do not even
really know what reproducibility means in this context?  Do you mean that if you run the exact same parameters your gun will work exactly the same way?  I do not think that is true -- isn't that what Table II is meant to demonstrate?  Do you mean reproduciblity of the BO?  In general, BO is reproducible if run in a deterministic fashion, but
generally is meant to be stochastic (and will not be reproducible).  I think you either need to retract this claim or better explain your definition of reproduciblity.

\textbf{Reply:}
We believe this comment is related to the previous one. In the particular case of thermal spray coating, we use the gun voltage as an indicator to the state of the equipment. The main reproducibility challenge is that when the input (control) parameters are set, the outputs are different for different measurement sessions. Finding a quantity that is not set in advance as the inputs, but correlates with the outputs, provides the opportunity to accommodate the changes or drifts in the equipment/process.
We integrate this measured quantity (voltage) as an additional modeling input to the coating quality (for microhardness in particular). When this is done, we achieve smaller uncertainly and higher predicting performance in modeling the coating properties. The same approach can be generalized to other processes, where a measurable quantity reflecting the state of the equipment/process can be included in the modeling of the output variables. We have modified the abstract according to the reviewer comment as well as to the new structure. \\

\textbf{Comment 8:} Your acquisition function and BO involves some interesting elements.  First, it seems like you are treating $S(\mathbf{x})$ as though it were free to compute.  If this is the case, it should probably be stated (since that
is the opposite of the standard assumption). 

\textbf{Reply:}
We appreciate this comment. The cost function $S(\mathbf{x})$ is indeed free to compute, being deterministic and known by the acquisition algorithm. We have clarified these statements further in sections \ref{sec_method} and \ref{sec_acquisition_procedure}.\\

\textbf{Comment 9:}
Another place where the algorithmic novelty is insufficiently demonstrated is in section \ref{sec_acquisition_procedure}.  "In preliminary experiments, we observed that acquisition procedures such as the one presented in \cite{Gardner2014BayesianConstraints} were too aggressive, while an approach focusing on FIP only led to excessively conservative exploration."	You just say this, and that's it.  In my opinion, if you are going to make this claim then you need to present results to that effect.  You can do that for the situation that you are working in, or on a manufactured problem (which would probably be preferable).  But without that, you are just saying something that the audience cannot verify, or even really place in their own context.

I would also like to see more analysis of your acquisition function in action, including with consideration of the pi value that appears (but for which we are not really given guidance on choosing).

\textbf{Reply:}
We sincerely thank the reviewer for their suggestion.
We have conducted simulated comparisons between our proposed method, its individual components (FIP and HFI) and the BO method that has been successfully applied to industrial applications \cite{Gardner2014BayesianConstraints}. The comparisons are summarized in Table \ref{tab_comparison} and commented in section \ref{sec_simulated_res}. We highlight that changing the value of $\pi$ corresponds to having a behavior more similar to FIP ($\pi=1$) or to HFI ($\pi=0$), as shown in Table \ref{tab_comparison}.\\

\textbf{Comment 10:}
I worry a bit about the fact that you fix 20000 points rather than conducting an actual optimization over the entire space, but I don't think that's the end of the world.

\textbf{Reply:}
We agree with the reviewer on the fact that other methods can be used to conduct the optimization of the acquisition function (such as particle swarm in continuous parameter spaces, that has been successfully applied to BO optimization of cascade PID controller parameters). Grid search with dense enough grids (which is the case here, with 20000 points) is however common practice as well. As the acquisition function optimization technique was not the focus of our work, we decided to use this simple and effective method.\\

\textbf{Comment 11:} The parameters that you were studying were all discrete: if I correctly understood section \ref{data_coll}, 6 parameters with 3 values and 2 parameters with 2 values, for a total of 2916 possible parametrizations of the experimental setup.  Is this correct?  If so, what are the 20000 candidates you describe creating in section \ref{sec_opt_workflow}?  Shouldn't there only be 2916?  If you mean to work in a continuous space, then when was your training/validation set created using a discrete domain?

\textbf{Reply:}
We thank the reviewer for raising this point. The input space $\mathcal{X}_\mathrm{c}$ is continuous. However, when collecting samples to create our training data set we necessarily had to discretize the space. Given the extremely high data collection cost, we used fractional factorial design to effectively expose the most important features of the process while respecting our evaluations budget. The validation set was created selecting combinations of inputs from the continuous space. Here, the discretization used for the training set was not followed. The validation set was chosen mostly based on expert considerations, again with the goal of limiting the number of experiments (which holds in realistic scenarios as well). Sections \ref{data_coll} and \ref{sec_mod_res} were modified to clarify data collection for the training and validation data sets respectively.\\

\textbf{Comment 12:}
I do not understand what is meant to be demonstrated in Figure \ref{fig_experimental_opt}. Why would you plot anything related to the "first optimization batch"?  Why would that be relevant?  Wouldn't you somehow want to either plot all of the feasible results or, simply, all of the results?  And why do you provide the 95\% prediction confidence?  What is that meant to
convey?  Is that a function of your models that you have built?  Aren't we actually taking real values from the gun at this point?  Why does it matter what your model says for a location where we actually have data?

And actually, at this point, I have a more confusing question -- did you run this for only a single BO iteration?  There does not seem to be any explanation of the actual results of your BO process, only the first batch (of which you cut one because you felt like it).  What epsilon did you use for these experiments that led you to conduct only
a single iteration?

\textbf{Reply:}
We thank the reviewer for asking these relevant questions. 
The very nature of the studied process did not allow us to conduct more BO iterations experimentally. Coating and analyzing each batch of samples can take up to three months. This made it impossible to conduct experiments until convergence was reached. Indeed, the results we show are all the experimental results that we could collect. We have clarified in section \ref{sec_exp_opt} that the interruption after batch one has been caused by time constraints. This is the reason why we put the focus on simulations, with whom the experiments are in agreement. 

Regarding the 95\% prediction confidence, the information is necessary to discuss the modeling uncertainty in the selected experimental locations (which we have now clarified). It highlights in particular the fact that there is larger uncertainty in microhardness due to the voltage offset. The most relevant information is indeed the real data that is indicated with black dots.
\\


\textbf{Comment 13:}
I also do not understand what Figure \ref{fig:detailed_opt} is.  Was this an actual experiment that was run?  Or is this just a demonstration of what something should look like?  If this is an actual experiment, why was it run to 4 batches when the other experiment was run for only a single batch?

\textbf{Reply:}
We appreciate this comment. We have clarified further in the text and in the section title, that Fig. \ref{fig:detailed_opt} details a \emph{simulated} optimization procedure. The APS process has been replaced with a neural network oracle that allowed us to conduct the presented study. On the other hand, Fig. \ref{fig_experimental_opt} contains the results of the real experiments that were conducted. As we explain in the text and in the previous reply, we could run all required experiments in the simulated cause (i.e. four batches) but could only run one batch in the experimental case. The modifications in the text and the section title, together with the changes made in section \ref{sec_exp_opt}, should clarify that the former contains simulations while the latter contains real data.

==> Reviews/Answer_to_reviewer_18.tex <==
\textbf{\large Reply to Reviewer 18:}\\\\
We thank the reviewer for their evaluation as well as their comments and suggestions on improving the quality of the manuscript.\\  


%----------------------------------------------------------------------
\textbf{Comment 1:}
This adapt this framework to the set-up and optimization of atmospheric plasma spraying processes. finally, validate a Gaussian process modeling structure to predict coatings properties. My suggestion is major revision

\textbf{Reply:}
We thank the reviewer for the summary and suggestion.\\

\textbf{Comment 2:}
It seems that the data are limited for GPR? is that suitable?

\textbf{Reply:}
Indeed, the data we have available for modeling are limited. The reason for this is that the experiments are extensive and the required quality evaluation is very time- and resource-intensive. We therefore propose methods that deal with this scarcity of data, both in training and in optimization trials.\\

\textbf{Comment 3:}
English should polished somehow

\textbf{Reply:}
We have worked to improve the paper, and have also conducted an extensive check, removing grammatical errors and typos.
\\

\textbf{Comment 4:}
Is it transferable to other processes?

\textbf{Reply:}
We appreciate this comment. As raised in the other reviews, transferability is an important point. We have therefore restructured the paper, and have highlighted the main contribution, which is the batch-BO with tailored acquisition functions. It can be applied to various manufacturing processes which are complex to conduct, expensive, slow, or require expensive evaluation to asses the achieved quality. Such processes are other types of plasma spray coating, such as VLPPS (very low pressure splasma spray) or additive manufacturing processes (selective laser melting, wire arc additive manufacturing, etc). The method's main benefit is that it achieves favorable configurations of parameters much faster than other methods, including those based on BO. 
The method's main benefit is that it achieves favorable configurations of parameters much faster than other methods, including those based on BO. This makes it possible to enable manufacturing of very small lots, without extensive simulations, time and experiments optimizing for the best parameters, which is one of the main goals in intelligent manufacturing. We have addressed these points in the introduction and, in particular, in the contributions of the paper. We believe this rearrangement and clarification has increased the value of the paper, and are very grateful to the reviewer for pointing this out.



==> Reviews_2/Answer_to_editor.tex <==
\textbf{\large Reply to the Editor:}\\


%----------------------------------------------------------------------
\textbf{Comment 1:}
In this review round, one reviewer, and the associate editor still believe that the algorithmic argument has not been sufficiently fleshed out with detailed evidence, and the contribution of the paper cannot reach the standard of the journal in such a short time for RA-L publication. An expansion of the applicability of the theory will allow for more convincing evidence of the benefits of this approach over other methods.

\textbf{Reply:}
Dear Prof. Popa,

We would like to thank you for the opportunity to resubmit our manuscript to RA-L, following the reviews and submission for CASE 2021.

The main contribution of this manuscript is a framework for the configuration and operation of expensive-to-evaluate advanced manufacturing methods, based on Bayesian optimization. We propose a method tailored towards sample efficiency, by designing custom acquisition functions. The method is applicable to a large class of manufacturing problems, relevant in advanced manufacturing. We include an experimental demonstration, optimizing the process parameters of a plasma spray coating process.

While the manuscript (ID 21-0855) was accepted for CASE 2021, one reviewer was still not convinced that the algorithmic argument has been sufficiently fleshed out with detailed evidence, which made the contribution of the paper insufficient to reach the standard of the journal in such a short time for RA-L publication. 

We therefore addressed these concerns, and also fully restructured the paper, and focused on the proposed approach, with less emphasis on its application. The paper has been completely re-written, with very little overlap with the conference paper. An expansion of the applicability of the theory allows for more convincing evidence of the benefits of this approach over other methods. In particular, we make our algorithmic approach more general and include an entirely new section where we study the method's performance thoroughly. We utilize three benchmark problems from the constrained optimization literature to compare Alg. 1 with a state-of-the-art method and support our contribution with detailed evidence. We also analyze our algorithm's performance as a function of the tunable hyper-parameter $\pi$. We believe that, thanks to the suggestions from the reviewers, we could present a much more complete and stronger work, demonstrating the benefits of our proposed approach. The paper is now suitable for a much wider audience as the main optimization algorithm (Alg. 1) has been tested on general optimization problems where it outperformed the most commonly used method. We have maintained a (shortened) section discussing experimental work (now updated with new experimental data) to support our claim that the algorithmic novelty we propose can be efficiently applied to a wide class of practical problems.

As the changes from the previous version have been significant, it was impossible for us to only highlight sentences to indicate minor changes and/or additions. In this re-submission, we have highlighted in \cmt{teal color} the titles of the existing sections that have been strongly restructured. We have then highlighted the entire Section IV as it is a completely new addition. Finally, we highlight Fig. 5 since it contains extra experimental data that were not present in the previous version.

==> Reviews_2/Answer_to_reviewer_19.tex <==
\textbf{\large Reply to Reviewer 19:}\\


%----------------------------------------------------------------------
\textbf{Comment 1:}
I recommend this submission for publication.  In this paper a GP model structure is used to predict coating properties, and an algorithm is proposed to enhance reproducibility in real-time process measurements. The experimental results the proposed method can efficiently find good configuration of APS process. The article is well organized and its presentation is good, and the citations is adequacy.

\textbf{Reply:}
We thank the reviewer.

==> Reviews_2/Answer_to_reviewer_20.tex <==
\textbf{\large Reply to Reviewer 20:}\\


%----------------------------------------------------------------------
\textbf{Comment 1:}
Accept

\textbf{Reply:}
We thank the reviewer.

==> Reviews_2/Answer_to_reviewer_21.tex <==
\textbf{\large Reply to Reviewer 21:}\\


%----------------------------------------------------------------------
\textbf{Comment 1:}
The revision has mostly addressed my main concerns with the paper, and I believe also most of the main concerns of other reviewers. The paper could still benefit of a more thorough experimental evaluation either in simulation or in a real-world scenario where comparisons with other methods are possible. However, the focus on the APS application in my view provides a representative application scenario. I would just suggest minor revisions on the text and the addition of suggestions for future work to the conclusion.

\textbf{Reply:}
We thank the reviewer for the comments and advice. The paper has now been completely restructured with a focus on the proposed optimization approach, and includes a thorough evaluation of the algorithm performance on benchmark problems using Monte Carlo methodology, that can be reproduced by the readers. We have also included additional experimental data to the APS application.
The manufacturing problem modeling and general detailed implementation has been described only in the conference paper.
\\

\textbf{Comment 2:}
The problem definition in Eq. 1 should be more general in terms of
the number of constraints. It should be reformulated in terms of "K"
constraints, as in Eq. 4.

\textbf{Reply:}
The problem definition (now Eq. 3) has been rewritten in its general form to include "K" constraints.
\\

\textbf{Comment 3:}
What are possible suggestions for future work? For example, can this
method scale to higher dimensions and large amounts of data? What if
the number of constraints to check is too large? Would the modelling of
any correlation between constraints provide prediction benefits?

\textbf{Reply:}
We appreciate the very relevant points raised by the reviewer. The possibility to scale Bayesian optimization methods to higher dimensions or large data sets is the object of numerous studies and we believe that the method we propose simply has the same known limitations that other similar approaches have.\\
Regarding the second point, outputs correlations have also been studied in general works both regarding Gaussian process modeling and Bayesian optimization (cf. Multitask Bayesian optimization). We certainly plan to investigate these methods deeper and in the context of our approach. However, because of space limitations, we could not include the future research directions in the conclusion of our paper.
\\

==> Reviews_2/Answer_to_reviewer_22.tex <==
\textbf{\large Reply to Reviewer 22:}\\


%----------------------------------------------------------------------
\textbf{Comment 1:}
I think that the revisions definitely present the topic more effectively to a broader audience. I still maintain my belief that, if this is actually meant to be an algorithm for broader usage, that there needs to be more extensive testing. The fact that the only testing taking place here is directly related to a problem that no one can run or reproduce makes me feel very uneasy and dissatisfied. And I'm more than a little concerned that the authors couldn't even manufacture some very trivial fake problems on which to test this. I generally consider that the minimum that is required in order to present an algorithm without any theoretical support (which, unless I'm mistaken, is missing).

\textbf{Reply:}
We thank the reviewer for the very relevant point. The paper has now been restructured, with a focus on the proposed optimization approach, and includes a thorough evaluation of the algorithm performance on benchmark problems using Monte Carlo methodology, that can be reproduced by the readers. We have also included additional experimental data to the APS application.
The manufacturing problem modeling and general detailed implementation has been described only in the conference paper.
\\

\textbf{Comment 2:}
Given that, there are certainly worse articles out there. Table II (authors' note: now Table III) is the absolute minimum acceptable comparison required for me to be okay with this. If this paper gets published, I certainly won't fight it and I'll be the first person testing this algorithm out (because I work on problems like this). But if this were submitted to INFORMS or SIAM or ICML I do not believe that it would not be accepted, and that is roughly the bar that I hold RA-L to.

\textbf{Reply:}
Given the presence of the new section (IV) where the algorithm's performance is evaluated on toy problems, Table III (that is specific to one application) is now supplemented by a broader study on different and reproducible conditions.
\\

\textbf{Comment 3:}
There are still things that I would like to better understand -- I might argue that going from 45\% to 48\% feasible samples is more important than an additional cost reduction from 103-102. I might say that 20\% (or even 17\%) is fine because I've gone from 102-101.	Can you argue otherwise? It's not obvious to me that you even tried to -- you simply said you prefer your algorithm. I would argue that Alg. 1, HFI, FIP all fall somewhere on the meta-Pareto Frontier of possible optimization strategies, with no obvious winner declared from Table II. You could even toss EI on there too if you want to include "familiarity" as a metric by which to judge the algorithms (since it performed similarly to HFI but is certainly much more well known).

\textbf{Reply:}
All the points raised by the reviewer are now discussed in Section IV, where the proposed algorithm is compared with the "familiar" EIC as well as with its components (HFI and FIP). Since the evaluations are conducted on multiple benchmark problems, the observations about performance on the APS simulation become less central. The trade-off between objective minimization and feasibility maximization is thoroughly discussed.
\\

\textbf{Comment 4:}
But, more importantly, can you argue otherwise on some other problem for some other person who tries to implement your algorithm? This is what I mean when I say that I think your paper needs more experimentation. I would love to see classes of constraints and objectives where Algorithm 1 is uniformly better, classes where HFI is comparable and classes where FIP does all the work. Maybe even some where EI is actually fine. I would also like some analysis of the implication of your various tunable parameters -- what is the implication of changing pi on the performance in different circumstances, and what guidance can you give your readers? If you are claiming to make an algorithmic contribution to the community I feel like that should be present.

\textbf{Reply:}
All the suggested experimentation is contained in Section IV. We thank the reviewer for this important suggestion that significantly improved the paper.
\\

\textbf{Comment 5:}
Can you identify a set of circumstances where your combination of HFI
and FIP is absolutely dominating of the other methods?	If not, that's
okay, but explain why not -- and do so as the result of extensive
experimentation and analysis of the types of circumstances where each
method excels (or fails). Without this, the results you are presenting
are not portable to any other set of circumstances. And, again, even
on this problem you have presented it's not obvious that your algorithm
is the "right" one, as someone who has a stronger preference for Cost
or \# Feasible would prefer one of the alternatives.

\textbf{Reply:}
In Section IV, we study the effect of the hyper-parameter $\pi$, that tunes the algorithm to select when HFI or FIP are used. In the study, we show how the combination of the two methods outperforms its individual components as well as EIC. We also explain how practitioners could select the best $\pi$ depending on their preferences.
\\


\textbf{Comment 6:}
I really like this idea of parametrizing the tradeoff between exploring
the feasible/satisfactory region and optimizing within it. This is an
important problem, but I feel like this paper is incomplete if it is
claiming to make an algorithmic contribution. I understand the
conflict between doing real work on an application and doing
algorithmic work on toy problems. But if you are not going to publish
in an application journal, then there needs to be some number of toy
problems or the reader is left unable to place this strategy in a
relatable context. And, it wouldn't hurt if there were at least 1 toy
problem (and, ideally, 1 class of problems) for which your Algorithm
dominates HFI and FIP.

\textbf{Reply:}
We agree with the reviewer on the important challenges posed by conducting algorithmic work on toy problems together with experimental work. In this second version of the paper we expanded the analysis of the proposed algorithm on benchmarks to show it indeed outperforms HFI and FIP on three problems taken from the literature. We also could compare Alg. 1 with known methods (EIC) to discuss the conditions under which the method we propose outperform the state-of-the-art technique for manufacturing parameters tuning.

==> Reviews_3/Answer_to_editor.tex <==
\textbf{\large Reply to the Editors:}\\


%----------------------------------------------------------------------
\textbf{Comment:}

This is a re-submission of a previously rejected paper. While the paper
has made some important improvements, the Reviewers and the Editors
think that the paper still needs substantial revisions before it can be
considered further for publication. 

Some major concerns include: the paper is difficult to follow; the main
contributions should be clarified and clearly established with respect
to the prior publication by the authors in IEEE CASE 2021 on plasma
spray process parameter optimization; and the experiments need to be
more thorough and convincing.
\\

\textbf{Reply:}

First we would like to thank the Editors and the Reviewers for the time and effort dedicated to our manuscript. We particularly appreciated the opportunity to resubmit this work, as it has been substantially improved from its first version.

We believe to have successfully addressed all the concerns expressed by the Reviewers.
The changes we have made to the manuscript also reflect the concerns raised by the Editors.
We have included a flow chart of the method (Fig. \ref{fig:flowchart}) that offers a visual representation of the proposed algorithms and clarifies the entire work, making the manuscript easier to follow. Additionally, multiple parts of the manuscript have been edited for added clarity.

We have highlighted and magnified the differences that exist between this manuscript and the previous submission in IEEE CASE 2021. The previously published work focused entirely on atmospheric plasma spraying (APS), for which we discussed at length data collection, modeling, simulation, and optimization experiments. While our optimization algorithm was introduced in IEEE CASE 2021, that formulation was exclusively tailored for APS and no algorithmic analysis of its performance on reproducible problems was provided. The contributions were entirely aimed at a very specific experimental context, lacking any theoretical performance analysis. In the current manuscript, instead, we have generalized the method for all advanced manufacturing applications (and optimization problems) and shifted the focus towards a solid, well-studied algorithmic contribution that is secondarily demonstrated on diverse applications. This reflects the suggestions received by the Editor and Reviewers at the time of rejection of the previous submission, and makes this work relevant to a very broad audience. The detailed study of Sec. \ref{sec:comparative_study} is one of the main contributions of this work, as readers can now compare the performance of our generalized BO algorithm with a state-of-the-art method on benchmarking problems from the literature, fully grasping the benefits and limitations of the proposed method. We now also study the effect of the hyper-parameter $\pi$ regulating the behavior of the algorithm, which allows practitioners to clearly understand how to tune our method for the desired performance on any problem. Furthermore, to reduce the overlap with IEEE CASE 2021, we strongly reduced the amount of content in Sec. \ref{sec_simulated_res}. After a careful analysis prompted by the Editors, we believe that Sec. \ref{sec:comparative_study} is sufficiently detailed and that the readers can refer to \cite{Guidetti_Plasma_BO} for additional details on APS configuration. 

We have included in this revised version more experimental data than it was previously available, making this manuscript much richer than the work published at IEEE CASE 2021 and offering the readers new and convincing experiments. Sec. \ref{sec_exp_opt} contains one additional batch of experiments that match the simulated study. We could unfortunately not conduct any other experiment on APS due to time and cost constraints. A new section (Sec. \ref{sec:FDM}) has been added to showcase the method on another completely different manufacturing process (i.e. 3D printing). We think these additional application fully highlights the performance of our method as well as the trade-off caused by hyper-parameter tuning.

We have highlighted all the changes that were made in \cmtb{teal color}.

==> Reviews_3/Answer_to_reviewer_1.tex <==
\textbf{\large Reply to Reviewer 1:}\\


%----------------------------------------------------------------------
\textbf{Comment 1:}
This revision is significant enough for me to feel that this paper
could be published in RA-L, now.  The authors have presented enough
experimentation to give guidance to the readers about their strategy
and its implications.

\textbf{Reply:}
We thank the Reviewer for the kind recommendation. We would like to thank them for all the comments received during the previous submission which helped us significantly improve this manuscript.
\\

\textbf{Comment 2:}
The manufactured problems (depicted in Figure 1) are, certainly, common
ones in the black-box constraint community and logical benchmarks for
comparison to other constrained black-box optimization problems. I
wonder, though, how closely constraints of this rather elaborate form
actually appear in practical circumstances.  It's possible that it is
quite common, but my hunch is there are also many circumstances where
the constraints produce a single, simple (maybe even convex) region of
feasibility within which the optimization actually takes place. 
Probably more like P2 than P1 or P3.  When I go to test this algorithm
(which I will be excited to do once this is accepted), I will be
working on problems which tend to look like that.  As a bit of a
suggestion for a future paper: the authors could consider what
modifications/adaptations can be made to their algorithm to best
leverage the belief that there is one contiguous feasible portion of
the domain.

\textbf{Reply:}
We agree with the Reviewer on the possibility that many real optimization problems might have simpler constraint sets. We chose to benchmark our method on problems from the literature that are considered challenging, to produce a detailed study of the algorithmic contribution and based on the idea that some of the applications we worked on (notably APS) have tremendously complex constraints. We nonetheless share the opinion that an extension targeted at simpler constraints set would be interesting.
\\

\textbf{Comment 3:}
Beyond that, I still don't love the low batch-count style experiments
-- how much can really be learned by any intelligent modeling with such
a small amount of data?  In my mind, the success is contingent almost
entirely on how good the GP prior beliefs are.	But, that's something
upon which the reader can opine: there are certainly many applications
which are as sample-sparse as is tested here.

\textbf{Reply:}
We agree that the restricted amount of available batches makes it hard to demonstrate experimentally the value of our method. Unfortunately, despite trying to do so, we could not conduct any extra experiments on APS. We have however included one new section on FDM configuration (Sec. \ref{sec:FDM}). There, it was possible to conduct a much larger number of experiments and to study the effect of the confidence threshold $\pi$ in experiments. We also believe that one of the main contributions of this work lies in the detailed study of the proposed algorithm on benchmarking problems, which offers more details to the readers about the method's performance and can be considered as informative as the experimental work.
\\

\textbf{Comment 4:}
I want to thank the authors for presenting a clean analysis of the
results of their experimentation.  I know that it can be tempting to
hide any tests where your algorithm doesn't "win".  But I consider it
very valuable to show where (and why) your design decisions have had a
positive impact.  That's one of the reasons I'm good to accept this
paper.

\textbf{Reply:}
We thank the Reviewer for this comment and share their same view on experimental data integrity.
\\

\textbf{Comment 5:}
I'll throw in one more conceptual question -- do you think that the
expected value of the red and blue lines in Figure 3 is a continuous
function of pi?  The data that is presented doesn't show enough to
suggest anything, and you don't seem to hypothesize about it.  Just
curious.

\textbf{Reply:}
The question is a very interesting one, and despite having postulated about the possible answer we are currently not ready to make a hypothesis. We currently believe that the constraints structure might have an impact on the continuity, but it is probably too early to make any claim. It is however a research direction that we intend to investigate in the near future and we thank the Reviewer for the observation.

==> Reviews_3/Answer_to_reviewer_14.tex <==
\textbf{\large Reply to Reviewer 14:}\\


%----------------------------------------------------------------------
\textbf{Comments 1 and 2:}
The idea is innovative but the flow of the paper is difficult to follow for the reader and needs to be revised appropriately. Need to use some figures or flowcharts.\\
Please add a flowchart or figure to show how the proposed
method works. 

\textbf{Reply:}
We have added a flowchart summarizing the entire method (Fig. \ref{fig:flowchart}). We thank the Reviewer for the suggestion and believe this addition has significantly increased the clarity of the work.
\\

\textbf{Comment 3:}
The literature review part needs to be revised and add new literature related to the application. Also need to add the literature related to the different methods of comparison done by different people with some facts and figures.

\textbf{Reply:}
We believe that the most important literature about APS is included in the submitted work. The revised paper now contains one new case study on 3D printing, for which we added the relevant literature. We have also included more papers on process modeling and control in the introduction. Finally, regarding the comparison with the competing method on benchmark problems, the literature is presented in Sec. \ref{sec:comparative_study} (e.g. \cite{Gardner2014BayesianConstraints,Gramacy2016ModelingOptimization,Letham2017ConstrainedExperiments}) which contains detailed figures and tables about the performance of our method as well as the state-of-the-art one.
\\

\textbf{Comment 4:}
On page 2 what is lambda in equations 1 \& 2 ? Please provide the definition of each symbol used in the equations.

\textbf{Reply:}
We have clarified what $\lambda$ is in the text after eq. \eqref{eqn:CBO}. While eq. \eqref{eqn:x_next} does not contain $\lambda$, we still made sure that all quantities (e.g. $\mathcal{X}$) are well defined.
\\

\textbf{Comment 5:}
Can you explain how your proposed method is different from the other people's?

\textbf{Reply:}
We have clarified in Sec. \ref{sec_acquisition_procedure} what are the difference between the state-of-the-art methods and our approach, and underlined the fact that the switching between two acquisition functions (eq. \eqref{fip} and \eqref{hfi}) is novel. Additionally, we would like to point out that the entirety of Sec. \ref{sec:comparative_study} is dedicated to the comparison between our method and the most used existing one, highlighting strength and weaknesses of both.
\\

\textbf{Comment 6:}
On page 6 (A. Simulated Process Optimization) section you mention the used neural network. What is the architecture or structure of the NN model?

\textbf{Reply:}
We have clarified that exhaustive details about the used neural network model can be found in \cite{Guidetti_Plasma_BO}, which has a stronger experimental focus and is entirely devoted to APS. In the current work, we simply reuse the same modeling configuration with no modification.
\\

\textbf{Comment 7:}
How fast  (speed of execution) is your proposed method as compared to other available methods? Please provide some facts.

\textbf{Reply:}
We have added the requested information in Sec. \ref{sec:pi_study}. We would like to point out that the method is mainly designed for manufacturing applications. As such, the milliseconds-long execution time is generally negligible in comparison to each manufacturing and analysis process whose duration can range from minutes to multiple weeks.
\\

\textbf{Comment 8:}
How does the complexity of the model affect when the number of sub-operations increases or decreases? Is the number of sub-operations affect the accuracy of the proposed method also?

\textbf{Reply:}
The dimensionality of the  inputs and outputs used to train the GP surrogate model has a significant impact on the performance of BO methods. This is not something specific exclusively to the submitted work but generally true for all BO methods. Generally, increasing the dimensionality corresponds to requiring more samples to obtain high quality GP priors that BO can rely upon. For an identical number of samples, this will equate to a lower accuracy of the optimization procedure. As the problem is a general one and not specific to the proposed method, we have not made changes in the manuscript which already includes the most relevant references about GPs, their use amd their limitations (e.g. \cite{Rasmussen2006GaussianLearning}).
\\

\textbf{Comment 9:} Is the proposed approach performance affected, if the multi-nature data of sub-operation is fused for the prediction case? For example in AM case, we fused the different nature \& frequency of data for the quality prediction case. 

\textbf{Reply:}
If data of different nature (e.g. images, spectra, discrete values, continuous values, etc.) can be efficiently fused in the surrogate GP, predictions can certainly be improved without significantly impacting the computational cost. This is however not the main focus of the submitted manuscript that proposes a novel acquisition procedure for BO relying on very general GPs. The appropriate modeling of manufacturing processes through GP using heterogeneous and multi-scale data is certainly a challenging task that other authors have tackled. The Reviewer can find more detail about high-quality modeling of APS in \cite{Guidetti_Plasma_BO}, where this task is discussed in greater detail.
\\

\textbf{Comments 10 and 11:} Need to add more detail in the case study section to show the
strength of the proposed method. Please provide some facts and figures in terms of the
limitation of your proposed methods.

\textbf{Reply:}
The algorithmic value of the proposed method is discussed in detail in Sec. \ref{sec:comparative_study}, where it is compared to the most used concurrent method and its strengths and weaknesses are discussed. We have also added to the manuscript a new section on FDM configuration (Sec. \ref{sec:FDM}) that further illustrates the proposed method in the experimental context. Together with Sec. \ref{sec_plasma}, these sections analyze in detail the performance of our novel configuration method. The limitations are discussed at length: Sec. \ref{sec_plasma} highlights the issues cause by large batch sizes and limited availability data, while Sec. \ref{sec:pi_study} and \ref{sec:FDM} illustrate the trade-off induced by the selection of different values of $\pi$.


==> Reviews_3/Answer_to_reviewer_16.tex <==
\textbf{\large Reply to Reviewer 16:}\\


%----------------------------------------------------------------------
\textbf{Comment 1:} In the page 1, in the introduction, authors say “The standard
approach for process configuration and optimization is based on statistical principles.”, they should include references [a]-[d] which also consider optimization based on statistical principles.  
\begin{itemize}
    \item [a] The Regulation of an Electric Oven and an Inverted Pendulum,
Symmetry, Vol. 14, No. 4, 759, 2022.
\item [b] Modified Linear Technique for the Controllability and Observability
of Robotic Arms, IEEE Access, Vol. 10, 3366-3377, 2022.
\item [c] PI-Type Controllers and $\Sigma$-$\Delta$; Modulation for Saturated
DC-DC Buck Power Converters, IEEE Access, Vol. 9, pp. 20346-20357,
2021.
\item [d] Optimization of Sliding Mode Control to Save Energy in a SCARA
Robot, Mathematics, Vol. 9, No. 24, 3160, 2021.
\end{itemize}

\textbf{Reply:}
We thank the Reviewer for the suggestion. We have included references to [b] and [c], which we found to be the most relevant in the discussion.
\\
 
\textbf{Comment 2:} In the page 2, in the equation (3), authors should clarify if there is a special reason to select all the restrictions with the same structure.

\textbf{Reply:}
$c(x) \leq \lambda$ is an extremely general structure as no assumption is made on the complexity of $c(x)$. Any constrait function can be reformulated as $c(x) \leq \lambda$ and, for example, in Sec. \ref{sec:comparative_study} we use very non-linear constraints written in this formulation. We have clarified in the text that no assumption is made on the structure of $c(x)$.
\\

\textbf{Comment 3:} In the page 3, in the equations (7a), (7b), in the algorithm 1, authors presents a commutative algorithm between FIP and HFI, they should clarify in this is a new idea if this paper or if it is from a previous work.

\textbf{Reply:}
We clarified in the text that eq. \eqref{fip} and \eqref{hfi} as well as the entire switching strategy (Alg. \ref{alg_candsel}) are novel.
\\

\textbf{Comment 4:} In the page in the algorithm 2, authors should clarify if algorithm
2 has a relation with algorithm 1 or if it a other alternative to solve the same problem.

\textbf{Reply:}
The two algorithms are nested. Alg. \ref{alg_workflow} is an outer loop that runs Alg. \ref{alg_candsel} at each iteration of the for loop (this is explained in the text of Alg. \ref{alg_workflow}, specifically at line 11). We have included a flowchart of our method (Fig. \ref{fig:flowchart}) that explains the nested relationship between Alg. \ref{alg_workflow} and \ref{alg_candsel} and hope that this point has been clarified sufficiently.
\\

\textbf{Comment 5:} In the page 7, in the conclusion, authors should clarify if they
explain some future research. 

\textbf{Reply:}
The conclusion summarizes the paper, and does not present future research. We have clarified this by rephrasing some sentences to make the contents more evident. Due to space limitations we could unfortunately not include future research directions in the conclusion of this manuscript.


==> Reviews_summary.tex <==
Major issues:
Major points:


- Experiments provide no comparisons against baseline methods. The modelling component of the proposed framework is assessed in terms of predictive power against real data. The optimisation component, however, an essential part of the paper's main contribution is not compared against other methods. Therefore, it is hard to judge whether the proposed BO framework offers real performance improvements against existing out-of-the-box constrained BO methods (e.g., [12]).
One could argue that experimental comparisons using the real APS system are too expensive to run, so that the results in Sec. VI-B are still acceptable. However, the numerical experiments in Sec. VI-A were performed using a neural network oracle, which should much cheaper to evaluate, allowing for comparisons against other BO methods as baselines.

- the strategy that you used and the results of your paper are only relevant to your exact problem (which is so secretive that you couldn't even explain completely what it is).  That can be fine, but I have no perspective of the significance of the modeling results presented in Figures 2 & 3, nor the BO results presented in Figures 4 & 5.	Frankly, I don't know what fraction of the RA-L audience is going to understand how difficult it is to achieve your goal to "find combinations of inputs producing coatings with microhardness ranging between 635HV and 675HV and porosity between 6\% and 8.2\% while minimizing the gun stress index."  And you do not present any competing methods to provide a frame of reference for readers.
- First, the algorithm is never compared against any alternatives, or even on any problems that anyone else in the world can run (given your confidentiality).  How can the significance of your work be judged in such a vacuum? Second, you have done a significant amount of work to develop modeling strategies which are, possibly, only relevant for this specific application.  If you want to argue that there is an algorithmic contribution, don't you need to test this algorithm more broadly and see when it performs well and when it does not?
Essentially, my main problem is that this article wants to focus on a specific application but is trying to present a result as being more general than is demonstrated.  Either a number of more general tests need to be run to make an actual statement about your algorithm, or you should publish this in a forum where people can understand your application, and then more specifically explain the significance of this previously unachieved performance.
- Another place where the algorithmic novelty is insufficiently demonstrated is in section IV-A.  "In preliminary experiments, we observed that acquisition procedures such as the one presented in [12] were too aggressive, while an approach focusing on FIP only led to excessively conservative exploration."	You just say this, and that's
it.  In my opinion, if you are going to make this claim then you need to present results to that effect.  You can do that for the situation that you are working in, or on a manufactured problem (which would probably be preferable).  But without that, you are just saying something that the audience cannot verify, or even really place in their own context.

- Beyond that, I am very concerned about the distribution of the Validation values relative to the Training values.  When I think about the training/validation split in surrogate modeling, I think that the goal is for the training and validation sets to somehow be drawn from the same distribution.	The fact that the red squares seem to occupy only a fraction of the region that the blue dots occupy makes me worried that they do not belong to the same distribution.  As a result, it makes me somewhat concerned about how effective these GP models are, and in turn how much your algorithm actually relies on them (assuming the algorithm is performaing well).
Your strategy for creating this validation set was arbitrary, and not at all reproducible (given the expertise required), so this is part of my concern about suggesting a signficant algorithmic novelty in this article.

- I would also like to see more analysis of your acquisition function in action, including with consideration of the pi value that appears (but for which we are not really given guidance on choosing).




Relevant observations:

- The results in Figure 2 seem a bit troubling to me. First, you said that you created 86 pieces of data for your training set and 23 pieces of data for your validation set.  When I look at the Porosity graph, I count only 15 red squares.  Am I misunderstanding where the 23 is being used, or are there just some squares that happen to lie exactly on top of each other?	If there are, that seems a bit odd, right, given your statement in Table II about how much noise is affecting the accumulation of data?

- There is some missing detail about the modelling of the constraints. Are each of the constraints (c_1 and c_2) modelled with an independent GP? Or are they jointly modelled by a vector-valued GP?

- There is a lack of the explanation of whether collected training data set are able to cover regression feature-space effectively? If it is ineffective, the generalization ability is limited without high accuracy of prediction for those sufficient distant data points.

- In the subsection of Modeling Validation, an explanation of why the selected five combinations have the highest confidence should be provided. 

- Along these lines, I worry about this voltage discussion.  First, Figure 3 seems to present a bizarre disconnect between the training and validation data; why did you use totally different methods to create the training and validation datasets?  Why not use the exact same strategy for both?  Second I can read the Section IV-C and somewhat understand how you are incorporating voltage, but not really. And it should not matter if the focus is on the algorithmic side (since this strategy would not be applicable in any other settings).  The comment "voltage cannot be ... optimized" feels false as well.	If I understand, voltage is a function of your tunable parameters. How would optimizing it be any different than optimizing any other black-box function (which is what BO is built to do)?

- In your abstract you claim "We ... propose an algorithm that adapts to real-time process measurements to improve reproducibility."	I do not feel that you have done that anywhere in the paper.  I do not even really know what reproducibility means in this context?  Do you mean that if you run the exact same parameters your gun will work exactly the same way?  I do not think that is true -- isn't that what Table II is meant to demonstrate?  Do you mean reproduciblity of the BO?  In general, BO is reproducible if run in a deterministic fashion, but generally is meant to be stochastic (and will not be reproducible).  I think you either need to retract this claim or better explain your definition of reproduciblity.

- Your acquisition function and BO involves some interesting elements. First, it seems like you are treating S(x) as though it were free to compute.  If this is the case, it should probably be stated (since that is the opposite of the standard assumption).




Not too relevant observations:

- Gaussian process regression (GPR) is used to predict coating properties, its high computational complexity of both large data points and high dimension (using all variables in Section of Method) limits the real-time application. An explanation of your tractable computation power should be provided.

- I worry a bit about the fact that you fix 20000 points rather than conducting an actual optimization over the entire space, but I don't think that's the end of the world.

- The parameters that you were studying were all discrete: if I correctly understood section V-A, 6 parameters with 3 values and 2 parameters with 2 values, for a total of 2916 possible parametrizations of the experimental setup.  Is this correct?  If so, what are the 20000 candidates you describe creating in section IV-C?  Shouldn't there only be 2916?  If you mean to work in a continuous space, then when was your training/validation set created using a discrete domain?

- I do not understand what is meant to be demonstrated in Figure 5. Why would you plot anything related to the "first optimization batch"? Why would that be relevant?  Wouldn't you somehow want to either plot all of the feasible results or, simply, all of the results?  And why do you provide the 95\% prediction confidence?  What is that meant to convey?  Is that a function of your models that you have built?  Aren't we actually taking real values from the gun at this point?  Why does it matter what your model says for a location where we actually have data?
And actually, at this point, I have a more confusing question -- did you run this for only a single BO iteration? There does not seem to be any explanation of the actual results of your BO process, only the first batch (of which you cut one because you felt like it).  What epsilon did you use for these experiments that led you to conduct only a single iteration?
I also do not understand what Figure 4 is.  Was this an actual experiment that was run?  Or is this just a demonstration of what something should look like?  If this is an actual experiment, why was it run to 4 batches when the other experiment was run for only a single batch? 

